Understanding Driver Agency in RideSharing

Agency is an important human characteristic that users of automated complex technologies are usually denied. This affects the user's experience leading to decreased satisfaction and productivity. In this paper, we consider the ridesharing context and interviewed 7 drivers to understand the controls that would improve the agency they feel. The results show that they desire transparency, community and an effective ability to seek redress.

==> 0-TODO_LIST.tex <==
%TC:ignore
\noindent

Version: \DTMnow{} $\approx$
9661
words \hfill \reportOnFIXME

{\footnotesize
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}
\tableofcontents
%\listoftables
%\listoffigures
}

\textbf{\LARGE{TODO\_LIST}}
\begin{enumerate}

\item There are a few peculiarities about the organization of this.
First, ensure that the MAIN .tex and the .bib are ON THE TOP LEVEL AND NAMED THE SAME THING. 
Failure to do so will make submission to arXiv via automatically download/uploading more complicated. 
The rest of this file is just some example formattings from old files.

\end{enumerate}


\textbf{\LARGE{TODO-LIST}}
\begin{enumerate}

\item do the thing

\end{enumerate}

\newpage
\setcounter{page}{1}
%TC:endignore

==> documentBody/a-leftovers.tex <==
\section{LEFTOVERS}

I recommend keeping this file around to collect stuff that was ``well written, but not in the right part of the story''
